Variational Autoencoder for Generating Broader-Spectrum prior Proposals in Markov chain Monte Carlo Methods

This study uses a Variational Autoencoder method to enhance the efficiency and applicability of Markov Chain Monte Carlo (McMC) methods by generating broader-spectrum prior proposals. Traditional approaches, such as the Karhunen-Lo\`eve Expansion (KLE), require previous knowledge of the covariance function, often unavailable in practical applications. The VAE framework enables a data-driven approach to flexibly capture a broader range of correlation structures in Bayesian inverse problems, particularly subsurface flow modeling. The methodology is tested on a synthetic groundwater flow inversion problem, where pressure data is used to estimate permeability fields. Numerical experiments demonstrate that the VAE-based parameterization achieves comparable accuracy to KLE when the correlation length is known and outperforms KLE when the assumed correlation length deviates from the true value. Moreover, the VAE approach significantly reduces stochastic dimensionality, improving computational efficiency. The results suggest that leveraging deep generative models in McMC methods can lead to more adaptable and efficient Bayesian inference in high-dimensional problems.

==> domain.tex <==

%\documentclass[tikz]{standalone}
%\usepackage{graphicx} % Required for inserting images
%\usepackage{color}
%\usetikzlibrary{arrows.meta}
%\usepackage{amsfonts}
%
%\begin{document}

%\input{macros}
%\pagestyle{empty}
\begin{tikzpicture}[>=latex,scale=1]

\pgfmathsetmacro{\nodescale}{0.7}
\pgfmathsetmacro{\crad}{0.075}
\pgfmathsetmacro{\atop}{0.18}
\pgfmathsetmacro{\abot}{-0.13}

\draw[step=0.12,thin,help lines,draw=gray!10] (-3,-3) grid (3,3);

\draw[draw=red,line width=1,-{Stealth[scale=0.5]}] (-0.15,-0.15) -- (0.2,0.2);
\draw[draw=red,fill=white,line width=1] (0,0) circle (1.1*\crad);

\foreach \x in {1,2,...,49}{
    \draw[draw=black] (-3+0.12*\x,-3)--(-3+0.12*\x,-2.95);
    \draw[draw=black] (2.95,-3+0.12*\x)--(3,-3+0.12*\x);
    \draw[draw=black] (-3+0.12*\x,2.95)--(-3+0.12*\x,3);
    \draw[draw=black] (-3,-3+0.12*\x)--(-2.95,-3+0.12*\x);
}
\foreach \x in {1,2,3}{
    \draw[draw=black] (-3+1.5*\x,-3)--(-3+1.5*\x,-2.9);
    \draw[draw=black] (2.9,-3+1.5*\x)--(3,-3+1.5*\x);
    \draw[draw=black] (-3+1.5*\x,2.9)--(-3+1.5*\x,3);
    \draw[draw=black] (-3,-3+1.5*\x)--(-2.9,-3+1.5*\x);
}
\foreach \x in {1,2,3,4,5}{
    \node[scale=\nodescale] at (-3.6+1.2*\x,-2.4){+};
    \node[scale=\nodescale] at (-3.6+1.2*\x,-1.2){+};
    \node[scale=\nodescale] at (-3.6+1.2*\x,0){+};
    \node[scale=\nodescale] at (-3.6+1.2*\x,1.2){+};
    \node[scale=\nodescale] at (-3.6+1.2*\x,2.4){+};
    \node[scale=\nodescale] at (-3+1.5*\x-1.5,-3.3){\pgfmathparse{(\x-1)*25}\pgfmathprintnumber[fixed,precision=1]{\pgfmathresult}};
    \node[scale=\nodescale] at (-3.35,-3+1.5*\x-1.5){\pgfmathparse{(\x-1)*25}\pgfmathprintnumber[fixed,precision=1]{\pgfmathresult}};
}

\draw (-3,-3) rectangle (3,3);

\draw[draw=red,line width=1] (0,0) circle (1.1*\crad);

\draw[draw=blue,line width=1,-{Stealth[scale=0.5]}] (\abot-3,\abot-3) -- (\atop-3,\atop-3);
\draw[draw=blue,fill=blue,line width=1] (-3,-3) circle (\crad);
\draw[draw=blue,line width=1,-{Stealth[scale=0.5]}] (\abot-3,\abot+3) -- (\atop-3,\atop+3);
\draw[draw=blue,fill=blue,line width=1] (-3,3) circle (\crad);
\draw[draw=blue,line width=1,-{Stealth[scale=0.5]}] (\abot+3,\abot+3) -- (\atop+3,\atop+3);
\draw[draw=blue,fill=blue,line width=1] (3,3) circle (\crad);
\draw[draw=blue,line width=1,-{Stealth[scale=0.5]}] (\abot+3,\abot-3) -- (\atop+3,\atop-3);
\draw[draw=blue,fill=blue,line width=1] (3,-3) circle (\crad);

\draw[draw=blue,line width=0.5,-{Stealth[scale=0.75]}] (3,-0.5) -- (3.5,-0.5);
\node[scale=\nodescale,above] at (3.25,-0.5){$\vetor{n}$};

%\draw[draw=blue,line width=0.5,-{Stealth[scale=0.75]}] (3,0.5) arc (-90:0:0.25);
\draw[draw=blue,line width=0.5,-{Stealth[scale=0.75]}] (3,0.5) -- (3.5,0.5) -- (3.5,0.75);
\node[scale=\nodescale,above] at (3.5,0.75){$\Domb$};
\node[scale=\nodescale] at (-1.8,1.8){$\Dom$};
\node[scale=\nodescale] at (0,-3.7){$x(m)$};
\node[scale=\nodescale,rotate=90] at (-3.8,0){$y(m)$};
\draw[draw=white] (3.8,-2) -- (3.8,2);

\end{tikzpicture}

%\end{document}

==> vae_diagram2.tex <==
%\documentclass[tikz,12pt]{standalone}
%\usepackage{graphicx} % Required for inserting images
%\usepackage{color}
%\usetikzlibrary{arrows.meta}
%\usepackage{amsfonts}
%
%\begin{document}
%
%\pagestyle{empty}
\begin{tikzpicture}[>=latex,scale=1]

%\node at (0,0) {\includegraphics[scale=1]{vae.pdf}};

\definecolor{mygreen}{RGB}{155, 208, 103};
\definecolor{myred}{RGB}{246, 170, 144};
\definecolor{myblue}{RGB}{186, 223, 218};
\definecolor{mygreen2}{rgb}{0,0.5,0};
\definecolor{myblue2}{rgb}{0.39, 0.58, 0.93};
\pgfmathsetmacro{\nodescale}{0.7}

\setlength{\fboxsep}{0pt}
\setlength{\fboxrule}{0.3pt}
%\input{macros}
%\draw[rounded corners=3,line width=0.7] (-7,-2.5) rectangle (7,2.5);

\draw[rounded corners=3,line width=0.7,fill=myblue2!50,draw=myblue2!110] (-7.1,-2.2) rectangle (-4.1,2.2);
\node at (-5.9,-2*0.15) {\fbox{\includegraphics[width=2cm]{vae_diagram/y4.png}}};
\node at (-5.75,-0.15) {\fbox{\includegraphics[width=2cm]{vae_diagram/y3.png}}};
\node at (-5.6,0) {\fbox{\includegraphics[width=2cm]{vae_diagram/y2.png}}};
\node at (-5.45,0.15) {\fbox{\includegraphics[width=2cm]{vae_diagram/y1.png}}};
\node at (-5.3,2*0.15) {\fbox{\includegraphics[width=2cm]{vae_diagram/y0.png}}};
\node[scale=\nodescale] at (-5.6,1.8)[align=center] {Input data};
\node[scale=\nodescale] at (-5.6,-1.8)[align=center] {$\dataset{X}$};
\draw[-{Stealth},line width=0.7] (-4,0) -- (-3.6,0);

\draw[rounded corners=1,line width=0.7,fill=mygreen!50,draw=mygreen] (-3.5,1.4) -- (-3.5,-1.4) 
               -- (-1.6,-0.7)
               -- (-1.6,0.7) -- cycle;
\node[scale=\nodescale] at (-2.55,0)[align=center] {Probabilistic \\[-2.5mm] encoder};
%\node[scale=\nodescale] at (-2.05,-0.35) {$\encoder_{\eparam}(x) \sim \fq{\ls|\datael{x}}$};
\draw[-{Stealth},line width=0.7] (-1.5,0) -- (-1.2,0) -- (-1.2,1) -- (-0.9,1);
\draw[-{Stealth},line width=0.7] (-1.5,0) -- (-1.2,0) -- (-1.2,-1) -- (-0.9,-1);

\draw[rounded corners=1,line width=0.7,fill=mygreen!50,draw=mygreen] (-0.8,0.6) rectangle (-0.4,1.4);
\draw[rounded corners=1,line width=0.7,fill=myred!40,draw=myred!75] (-0.8,-0.4) rectangle (-0.4,0.4);
\draw[rounded corners=1,line width=0.7,fill=mygreen!50,draw=mygreen] (-0.8,-1.4) rectangle (-0.4,-0.6);
\node[scale=\nodescale] at (-0.6,1) {$\me{\ls}$};
\node[scale=\nodescale] at (-0.6,0) {$\varepsilon$};
\node[scale=\nodescale] at (-0.6,-1) {$\desv{\ls}$};

\draw[-{Stealth},line width=0.7] (-0.3,1) -- (0,1) -- (0,0) -- (0.3,0);
\draw[-{Stealth},line width=0.7] (-0.3,-1) -- (0,-1) -- (0,0) -- (0.3,0);
\draw[-{Stealth},line width=0.7] (-0.3,0) -- (0.3,0);

\draw[rounded corners=1,line width=0.7,fill=myred!50,draw=myred] (0.4,-0.4) rectangle (0.8,0.4);
\node[scale=\nodescale] at (0,2)[align=center] {Sampled latent \\[-2.5mm] variable};
\node[scale=\nodescale] at (0.6,0) {$\ls$};
%\node at (0,-1) {\includegraphics[width=0.9cm]{gaussian_plot.png}};
\node at (0.6,-0.8) {\includegraphics[width=0.7cm]{vae_diagram/gaussian_python.png}};
%\node[scale=\nodescale] at (0,-2.25) {$ \ls = \me{\ls} + \desv{\ls} \varepsilon$};
%\node[scale=\nodescale] at (0,-2.75) {$\varepsilon \sim \normalf{0}{1}$};

\draw[-{Stealth},line width=0.7] (0.9,0) -- (1.5,0);
\draw[rounded corners=1,line width=0.7,fill=myblue!75,draw=myblue!125] (3.5,1.4) -- (3.5,-1.4) 
               -- (1.6,-0.7)
               -- (1.6,0.7) -- cycle;
\node[scale=\nodescale] at (2.55,0)[align=center] {Probabilistic \\[-2.5mm] decoder};
%\node[scale=\nodescale] at (2.05,-0.35) {$\decoder_{\dparam}(z) \sim \fp{\datael{x}'|\ls}$};

\draw[-{Stealth},line width=0.7] (3.6,0) -- (4,0);
\draw[rounded corners=3,line width=0.7,fill=myblue2!40,draw=myblue2] (4.1,-2.2) rectangle (7.1,2.2);
\node at (5.9,-2*0.15) {\fbox{\includegraphics[width=2cm]{vae_diagram/y4.png}}};
\node at (5.75,-0.15) {\fbox{\includegraphics[width=2cm]{vae_diagram/y3.png}}};
\node at (5.6,0) {\fbox{\includegraphics[width=2cm]{vae_diagram/y2.png}}};
\node at (5.45,0.15) {\fbox{\includegraphics[width=2cm]{vae_diagram/y1.png}}};
\node at (5.3,2*0.15) {\fbox{\includegraphics[width=2cm]{vae_diagram/y0.png}}};
\node[scale=\nodescale] at (5.6,1.8)[align=center] {Reconstructed data};
\node[scale=\nodescale] at (5.6,-1.8)[align=center] {$\dataset{X}'$};

\end{tikzpicture}

%\end{document}

